Asymptotic preserving IMEX-DG-S schemes for linear kinetic transport equations based on Schur complement

We consider a linear kinetic transport equation under a diffusive scaling, that converges to a diffusion equation as the Knudsen number $\varepsilon\rightarrow0$. In [3, 21], to achieve the asymptotic preserving (AP) property and unconditional stability in the diffusive regime with $\varepsilon\ll 1$, numerical schemes are developed based on an additional reformulation of the even-odd or micro-macro decomposed version of the equation. The key of the reformulation is to add a weighted diffusive term on both sides of one equation in the decomposed system. The choice of the weight function, however, is problem-dependent and ad-hoc, and it can affect the performance of numerical simulations. To avoid issues related to the choice of the weight function and still obtain the AP property and unconditional stability in the diffusive regime, we propose in this paper a new family of AP schemes, termed as IMEX-DG-S schemes, directly solving the micro-macro decomposed system without any further reformulation. The main ingredients of the IMEX-DG-S schemes include globally stiffly accurate implicit-explicit (IMEX) Runge-Kutta (RK) temporal discretizations with a new IMEX strategy, discontinuous Galerkin (DG) spatial discretizations, discrete ordinate methods for the velocity space, and the application of the Schur complement to the algebraic form of the schemes to control the overall computational cost. The AP property of the schemes is shown formally. With an energy type stability analysis applied to the first order scheme, and Fourier type stability analysis applied to the first to third order schemes, we confirm the uniform stability of the methods with respect to $\varepsilon$ and the unconditional stability in the diffusive regime. A series of numerical examples are presented to demonstrate the performance of the new schemes.

==> source/sec_introduction-v1.tex <==
\section{Introduction}
\label{sec:introduction}
Important physical phenomena like radiation transfer, neutron transport can be modeled by linear kinetic transport equations. 
We consider  a linear kinetic transport equation under a diffusive scaling:
\begin{align}
\label{eq:f_model}
\vareps \partial_t f + v\partial_x f = \frac{\sigma_s}{\vareps}(\lgl f \rgl - f) - \vareps \sigma_a f.
\end{align}
Here, $f(x,v,t)$ is the kinetic distribution function representing the phase probability density of particles, $x\in \Omega_x$ is the spatial position, $v\in \Omega_v$ is the velocity. $\sigma_s(x)\geq 0$ and $\sigma_a(x)\geq 0$ are the scattering and the absorption coefficients, respectively. $\lgl f \rgl =\int_{\Omega_v} f d\nu$ denotes the average of $f$ in the velocity space $\Omega_v$, where $\nu$ is a measure of the velocity space satisfying $\int_{\Omega_v}d\nu=1$. 
$\vareps>0$ denotes the Knudsen number, which is the ratio of mean free path of particles to the characteristic length.


The linear kinetic transport equation \eqref{eq:f_model} has a multiscale nature. With the assumption $\sigma_s>0$, as the Knudsen number $\vareps\rightarrow 0$, the kinetic transport equation will converge to the diffusion limit: 
\begin{align}
\label{eq:diffusion_limit_intro}
\partial_t \rho =  \lgl v^2\rgl \partial_{x}(\partial_x\rho/\sigma_s)-\sigma_a \rho,
\end{align}
where $\rho=\lgl f \rgl$ is the macroscopic density of particles. This multiscale nature poses computational challenges: (1) a standard explicit numerical scheme has a time step restriction $\Dt\leq O(\vareps h)$ ($h$ is the mesh size) due to stability, which is prohibitive in terms of computational cost for the diffusive regime with small $\vareps$; (2) when $\vareps$ is small,  an unconditionally stable implicit scheme, though not suffering from stability issue, may still fail to capture the correct physical limit on under resolved meshes \cite{caflisch1997uniformly,naldi1998numerical}.

The asymptotic preserving (AP) scheme \cite{jin2010asymptotic,degond2011asymptotic}, which preserves the asymptotic behavior of the physical model on the discrete level, is a natural candidate to conquer above challenges. As $\vareps\rightarrow 0$, an AP scheme solving \eqref{eq:f_model} will converge to a limiting scheme solving the diffusion limit \eqref{eq:diffusion_limit_intro}. As a result, it will be able to overcome the stability issue due to small $\vareps$ and capture the correct diffusion limit without resolving small $\vareps$ scale. AP schemes having explicit limiting schemes are considered in \cite{jin1998diffusive,klar1998asymptotic,jin2000uniformly,lemou2008new,liu2010analysis,jang2015high}. Due to the diffusive nature of the physical limit and the explicitness of the limiting schemes, these schemes have a parabolic time step restriction $\Dt= O(h^2)$ in the diffusive regime $\vareps\ll 1$. To enhance the stability, AP schemes with  implicit limiting schemes are developed in \cite{boscarino2013implicit,peng2019stability}. These schemes are unconditionally stable in the diffusive regime $\vareps\ll 1$.

To achieve unconditional stability in the diffusive regime, \cite{boscarino2013implicit} introduces a second reformulation to the even-odd decomposition \cite{jin2000uniformly} of \eqref{eq:f_model}. In \cite{peng2019stability}, a similar reformulation strategy is applied to the micro-macro decomposition \cite{liu2004boltzmann} of \eqref{eq:f_model}. Taking micro-macro decomposition as an example, a weighted diffusive term $\omega \partial_{x}(\partial_x\rho/\sigma_s)$, which is determined by the diffusion limit, is added to both sides of one equation in the decomposed system. Then, a suitable implicit-explicit (IMEX) Runge-Kutta (RK) time discretization is applied to the newly reformulated system. More specifically, the added diffusive terms $\omega \partial_{x}(\partial_x\rho/\sigma_s)$ on different sides of the equation are treated differently in the implicit-explicit strategy. In space, local discontinuous Galerkin (LDG) method is applied. The resulting IMEX-LDG scheme is AP and can be high order in time, and its limiting scheme is an implicit scheme solving the diffusion limit.  Based on Fourier analysis, \cite{peng2019stability} obtains the stability condition by numerically solving an eigenvalue problem, and confirms the unconditional stability in the diffusive regime. Furthermore, with energy analysis, in \cite{peng2020analysis}, the stability condition is rigorously achieved for the first order in time scheme.

In a multiscale problem, $\sigma_s(x)$ may vary spatially, and the diffusion dominant and transport dominant subregions may coexist. Despite the success of enhancing the stability in the diffusive regime, the further reformulation strategy also introduces two issues when solving these multiscale problems. First, the choice of the numerical weight is problem-dependent, and this ad-hoc choice has an influence on the performance of the numerical simulation. Second,  when the scattering coefficient $\sigma_s(x)$ varies spatially, intuitively, a spatially dependent weight function $\omega$ seems to be preferred to better capture the multiscale behavior. However, with such a spatial dependent weight, an extra non-physical assumption may be needed to maintain local conservation property, see Section \ref{sec:model} for more discussions. %Third, in the transport dominant regime with large $\vareps$, the real physical solution may lack regularity to guarantee $\partial_{x}(\partial_x\rho/\sigma_s)$ well-defined.

To overcome these issues and still accomplish unconditional stability in the diffusive regeime, we here design a new family of AP IMEX discontinuous Galerkin (DG) schemes \cite{cockburn2012discontinuous} based on the Schur-complement \cite{zhang2006schur}. Our new schemes directly solve the micro-macro decomposed system without any additional reformulation, hence, they do not suffer from issues mentioned above. 
In time, we apply high order IMEX-RK time integrators with a new implicit-explicit strategy. In space, we use DG discretization with a careful choice of numerical fluxes. In the velocity space, we consider a discrete ordinates method \cite{larsen2010advances}.  On the solver level, the key is to apply the Schur complement to the fully discrete system, which makes the computational cost on each time step comparable with \cite{peng2019stability}.  Furthermore, as $\vareps\rightarrow 0$, asymptotic analysis shows that our new schemes formally converge to high order in time local discontinuous Galerkin (LDG) methods \cite{cockburn1998local} solving the diffusion limit. Our new schemes are also more robust when an initial layer exists, hence, initial layer fix strategy in \cite{peng2019stability} is no longer needed.  Rigorous energy analysis for the first order scheme and Fourier analysis for high order schemes are presented to obtain the stability conditions. Uniform stability with respect to $\varepsilon$ and unconditional stability in the diffusive regime are verified by these analyses. Numerical examples are presented to demonstrate the performance of the IMEX-DG-S scheme and its advantage over the IMEX-LDG scheme.

The paper is organized as follows. In Section \ref{sec:model}, we briefly review the micro-macro decomposition, the further reformulation strategy in \cite{boscarino2013implicit,peng2019stability} and motivate the current paper. In Section \ref{sec:method}, we define our numerical schemes, and present the details of the Schur complement for the final matrix-vector system. In Section \ref{sec:AP}, formal asymptotic analysis is presented to confirm the asymptotic preserving property. In Section \ref{sec:stability}, energy and Fourier analyses are performed to obtain stability condition. In Section \ref{sec:numerical}, numerical results are presented to illustrate the performance of the new schemes. %In Section \ref{sec:conclusion}, concluding remarks are made.


==> source/sec_stability-v1.tex <==
\section{Stability}
\label{sec:stability}
In this section, numerical stability analysis will be carried out. An energy approach will be applied to the first order IMEX1-DG1-S scheme in Section \ref{sec:energy}, and Fourier analysis will then be applied to the first to the third order schemes, namely IMEX$k$-DG$k$-S scheme, $k=1, 2, 3$ in Section \ref{sec:fourier}.
%We will use IMEX$r$-DG$k$-S to refer to the fully discrete scheme with $r$-th order IMEX-RK time integrator and  $U_h^{k-1}$ discrete space in spatial discretization. Here S stands for the Schur complement. 
The analysis shows that our schemes are uniformly stable with respect to $\vareps$ and unconditionally stable in the diffusive regime.   Throughout this Section, we assume periodic boundary conditions in $x$, and $\sigma_s(x)\geq \sigma_m>0, \;\forall x\in \Omega_x$.

%When $\sigma_s=0$, $f$ is decoupled in the velocity space, and the system is transport dominant, so physically, $\vareps=O(1)$ where $\sigma_s=0$. Here, our main goal is to verify the unconditional stability in the diffusive regime $\vareps\ll1$. Hence, we assume $\sigma_s>0$ throughout this Section. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Energy analysis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Energy analysis for IMEX1-DG1-S scheme}
\label{sec:energy}

In this section, 
%\LL{For a general $\Omega_v$,
we will present an energy approach for stability analysis of
the IMEX1-DG1-S scheme \eqref{eq:full_first} for a general bounded $\Omega_v$. \BL{Without loss of generality, we assume the mesh is uniform with $h=h_i, \forall i$.} 
We first define  a  $\mu$-dependent discrete energy $E_{\mu,h}$ with $\mu\in[0,1]$ as a parameter. To guarantee $E_{\mu,h}$ non-increasing, we obtain $\mu$-dependent stability conditions. The results are further optimized with respect to $\mu$. The similar energy type stability analysis for higher order in time schemes is harder and left to our future investigation. 
%Then, we optimize solve an optimization problem to obtain an optimal stability condition independent of $\mu$. We want to mention that it is nontrivial to generalize this energy analysis to high order in time schemes.

Let $||\cdot||$ denote the standard $L^2$ norm for $L^2(\Omega_x)$. Define $|||g|||=\sqrt{\lgl(g,g)\rgl_h}$ and $|||g|||_s=\sqrt{\lgl (\sigma_s g,g)\rgl_h}$.
% With $\sigma_s\geq \sigma_m>0$, one can easily verify that $\forall \eta(x,v)\in L^2(\Omega\times\Omega_v;x\times\nu)$, $|||\eta|||\geq 0$ and $|||\eta|||_s\geq 0$.
In our  analysis, an inverse inequality is frequently used:  there exists a constant $C_{inv}=C_{inv}(l)>0$ such that
%\begin{subequations}
%\label{eq:inv}
\begin{align}
&|\phi(y)|^2 (b-a) \leq C_{inv}\int_a^b |\phi(x)|^2 dx, \quad\mbox{with}\; y=a \;\mbox{or}\; b,\;\;\;\forall \phi\in P^l([a,b]). \label{eq:inv:1}
%\\
%&(b-a)^2 \int_a^b |\phi'(x)|^2 dx \leq \widehat{C}_{inv}\int_a^b |\phi (x)|^2 dx.
%\label{eq:inv:2}
\end{align}
%\end{subequations}
Particularly, $C_{inv}(0)=1$. We also use Young's inequality: $xy\leq \theta y^2 +\frac{x^2}{4\theta},\; \forall \theta>0$.


\begin{defn}
\label{def:stab}
Given $\mu\in[0,1]$, we define a discrete energy for our schemes,
\begin{align}
\label{eq:mu:ene:def}
E_{\mu,h}^n=||\rho_h^n||^2+\vareps |||g_h^{n}|||^2+(1-\mu)\Dt|||g_h^n|||^2_s.
\end{align} 
The scheme is $\mu$-stable, if $E_{\mu,h}^{n+1}\leq E_{\mu,h}^n,\;\forall n\geq0$. If there exists $\mu\in[0,1]$ such that the scheme is $\mu$-stable, then the scheme is stable. If the scheme is stable (resp. $\mu$-stable) for arbitrary 
$\Dt>0$, then it is unconditionally stable (resp. $\mu$-stable).
\end{defn}

\begin{rem}
The $\mu$-dependent discrete energy $E_{\mu,h}^n$ in \eqref{eq:mu:ene:def} is quite different from that in  \cite{jang2014analysis, peng2020analysis}. Particularly,  the discrete energy in \cite{jang2014analysis, peng2020analysis} involves $\rho_h$ and $g_h$ from different time levels.
%which further leads to a different definition of $\mu$-stability (resp. stability) from \cite{peng2020analysis}.
\end{rem}

%%%%%%%%%%%%%%%%%%%%%%
% $\mu$-stability for IMEX1-DG1-S
%%%%%%%%%%%%%%%%%%%%%%
\begin{thm}[{\bf$\mu$-stability}]
%\textbf{($\mu$-stability)}
\label{thm:mu_stable}
Given $\mu\in[0,1]$, IMEX1-DG1-S scheme is unconditionally $\mu$-stable, if 
\begin{align}
\frac{\vareps}{\sigma_m h} \leq \lambda_0(\mu):=\frac{1-\mu}{2||v||_\infty}.
\label{eq:uncond-stable-region}
\end{align}
Otherwise, it is $\mu$-stable under the time step condition
\begin{align}
\Dt\leq\tau_0(\mu):=\frac{2\vareps^2 h}{2\vareps ||v||_\infty-(1-\mu)\sigma_mh}.\label{eq:CFL}
\end{align}
\end{thm}
%%%%%%%%%%%%%%%%%
% stability for IMEX1-DG1-S
%%%%%%%%%%%%%%%%
%\begin{thm}\textbf{(stability)}\label{thm:stable}
%The IMEX1-DG1-S scheme is unconditionally stable, if 
%\begin{align}
%\frac{\vareps}{\sigma_m h} \leq \frac{1}{2||v||_\infty}.
%\end{align}
%Otherwise, it is stable under the time step size condition
%\begin{align}
%\Dt\leq\frac{2\vareps^2 h}{2\vareps ||v||_\infty-\sigma_mh}.\label{eq:CFL}
%\end{align}
%\end{thm}
%%%%%%%%%%%%%%%%%%%%%%%%%%
% proof for $\mu$-stability for IMEX1-DG1 -S
%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proof}
%[{\bf Proof of Theorem  \ref{thm:mu_stable}. }]
%%%%%%%%%%%%%%

Take $\testR=\rho_h^{n+1}$ in \eqref{eq:full_first_rho}, and take $\testG=\vareps^2 g_h^{n+1}$ in \eqref{eq:full_first_g}. %substitute integral operator $\lgl \cdot\rgl$ with its discrete counterpart $\lgl\cdot \rgl_h$. 
Sum up \eqref{eq:full_first_g} for different collocation points $v_l$ with the corresponding weight $\omega_l$, we have 
\begin{subequations}
\begin{align}
&\frac{1}{\Dt}(\rho_h^{n+1}-\rho_h^n,\rho_h^{n+1})+l_h(\lgl vg_h^{n+1}\rgl_h,\rho_h^{n+1})\notag\\
=&\frac{1}{2\Dt}(||\rho_h^{n+1}||^2-||\rho_h^n||^2+||\rho_h^{n+1}-\rho_h^n||^2)+l_h(\lgl vg_h^{n+1}\rgl_h,\rho_h^{n+1}) 
=-(\sigma_a\rho_h^{n+1},\rho_h^{n+1}),
\label{eq:proof1-1}\\
&\frac{\vareps^2}{\Dt}\lgl(g_h^{n+1}-g_h^n,g_h^{n+1})\rgl_h+\vareps \lgl b_{h,v}(g_h^n,g_h^{n+1})\rgl_h-\lgl vd_h(\rho_h^{n+1}, g_h^{n+1})\rgl_h\notag\\
=&\frac{\vareps^2}{2\Dt}(|||g_h^{n+1}|||^2-|||g_h^n|||^2+|||g_h^{n+1}-g_h^n|||^2)+\vareps\lgl b_{h,v}(g_h^n,g_h^{n+1})\rgl_h
-d_h(\rho_h^{n+1}, \lgl vg_h^{n+1}\rgl_h)\notag\\
=&  -|||g_h^{n+1}|||_s^2-\varepsilon^2\lgl (\sigma_a g_h^{n+1},g_h^{n+1})\rgl_h.
\label{eq:proof1-2}
\end{align}
\end{subequations}

Summing up \eqref{eq:proof1-1} and \eqref{eq:proof1-2}, with Lemma \ref{lem:adjoint_relation}, we obtain
\begin{align}
&\frac{1}{2\Dt}( ||\rho_h^{n+1}||^2+\vareps^2|||g_h^{n+1}|||^2-||\rho_h^n||^2-\vareps^2|||g_h^n|||^2)
+\frac{1}{2\Dt}(||\rho_h^{n+1}-\rho_h^n||^2+\vareps^2|||g_h^{n+1}-g_h^n|||^2)
\notag\\
&+(\sigma_a\rho_h^{n+1},\rho_h^{n+1})+\varepsilon^2\lgl (\sigma_a g_h^{n+1},g_h^{n+1})\rgl_h+|||g_h^{n+1}|||_s^2\notag \\
&+\vareps
\lgl b_{h,v}(g_h^n-g_h^{n+1},g_h^{n+1})\rgl_h+\vareps\lgl b_{h,v}(g_h^{n+1},g_h^{n+1})\rgl_h
=0.
%\lgl b_{h,v}(g_h^n,g_h^{n+1})\rgl_h=0.
\label{eq:proof1}
\end{align}
Similar to \cite{peng2020analysis}, we split $|||g_h^{n+1}|||_s^2$ into 
\begin{align}
\label{eq:proof_split}
|||g_h^{n+1}|||_s^2
=\mu|||g_h^{n+1}|||_s^2+ (1-\mu)\Big(\frac{1}{2}|||g_h^{n+1}|||_s^2-\frac{1}{2}|||g_h^{n}|||_s^2
+\frac{1}{4}|||g_h^{n+1}-g_h^{n} |||_s^2 + \frac{1}{4}|||g_h^{n+1}+g_h^{n} |||_s^2\Big).
 \end{align}
%We split $\lgl b_{h,v}(g_h^n,g_h^{n+1})\rgl_h$ as $\lgl b_{h,v}(g_h^n-g_h^{n+1},g_h^{n+1})\rgl_h+\lgl b_{h,v}(g_h^{n+1},g_h^{n+1})\rgl_h$. 
With the piecewise constant in the discrete space, 
%Since piecewise constant polynomials are applied for the spatial discretization, 
$\partial_x g_h^{n+1}=0$. 
Following similar steps as in \cite{jang2014analysis} (such as its equation (3.22) and (3.24)), using the property of the solution in \eqref{eq:g:prop}, Young's inequaliy and the inverse inequality,  we obtain %the following estimates (see equation (3.22) and (3.24) in \cite{jang2014analysis} for details):
\begin{align}
&\lgl \bh(g_h^{n+1},g_h^{n+1})\rgl_h =\left\lgl\sum_i\frac{|v|}{2}[g_h^{n+1}]_\iL^2 \right\rgl_h,\label{eq:upwind}\\
&\left| \lgl \bh(g_h^{n+1}-g_h^{n} ,g_h^{n+1}) \rgl_h \right|\leq \eta |||g_h^{n+1}-g_h^{n}|||^2+\BL{\frac{C_{inv} }{\eta h}}\sum_i \left\lgl (\frac{|v|}{2}[g_h^n]_\iL)^2\right \rgl_h.
%&\left| \lgl \bh(g_h^{n+1}-g_h^{n} ,g_h^{n+1}) \rgl_h \right|\leq \eta |||g_h^{n+1}-g_h^{n}|||^2+\frac{C_{inv} }{2\eta h}\sum_i \left\lgl (\frac{|v|}{2}[g_h^n]_\iL)^2\right \rgl_h.
%&\leq (\frac{\theta}{\sigma_m}+\eta) |||g_h^n-g_h^{n-1}|||^2 +\frac{\widehat{C }_{inv}  ||v^2||_\infty}{4\theta h^2} \left(\sigma_m ||| g_h^n|||^2\right) +\frac{C_{inv} ||v||_{\infty} }{2\eta h}\left\lgl \frac{|v|}{2}\sum_i [g_h^n]_\iL^2  \right\rgl
%\notag\\
%&\leq(\frac{\theta}{\sigma_m}+\eta) |||g_h^n-g_h^{n-1}|||^2 +\frac{\widehat{C }_{inv}  ||v^2||_\infty}{4\theta h^2} |||g_h^n|||_s^2
%+\frac{C_{inv} ||v||_{\infty} }{2\eta h}\left\lgl \frac{|v|}{2}\sum_i [g_h^n]_\iL^2  \right\rgl,
\label{eq:upwind_jump}
\end {align}
Here, $\eta$ is a positive parameter, which will be determined later.

Substitute \eqref{eq:proof_split}-\eqref{eq:upwind_jump} into \eqref{eq:proof1}, and utilize $\sigma_a\geq 0$, we get
\begin{align}
&\frac{1}{2\Dt}( E_{\mu,h}^{n+1}-E_{\mu,h}^n)+\frac{1}{2\Dt}||\rho_h^{n+1}-\rho_h^n||^2
+(\frac{\vareps^2}{2\Dt}+\frac{1-\mu}{4}\sigma_m - \vareps\eta)|||g_h^{n+1}-g_h^n|||^2\notag\\
&+\frac{1-\mu}{4}|||g_h^{n+1}+g_h^n|||_s^2+\mu|||g_h|||_s^2+\vareps(1-\frac{C_{inv}||v||_\infty}{2\eta h})\lgl \sum_{i}\lgl\frac{|v|}{2}[g_h^{n+1}]^2\rgl_h
\leq 0.
\end{align}

In order to guarantee $E_{\mu,h}^{n+1}\leq E_{\mu,h}^n$, we require 
\begin{subequations}
\begin{align}
&\frac{\vareps^2}{2\Dt}+\frac{1-\mu}{4}\sigma_m - \varepsilon\eta\geq 0,\label{eq:proof_l3.a}\\
&1-\frac{C_{inv}||v||_\infty}{2\eta h}\geq 0.\label{eq:proof_l3}
\end{align}
\end{subequations}
We choose $\eta=\frac{\vareps}{2\Dt}+\frac{1-\mu}{4\vareps}\sigma_m$, so \eqref{eq:proof_l3.a} holds. With $C_{inv}(0)=1$, the inequality in \eqref{eq:proof_l3} becomes
\begin{align}
&\frac{\vareps}{\Dt}\geq\frac{2||v||_\infty\vareps-(1-\mu)\sigma_mh }{2\vareps h}.\label{eq:proof_final}
\end{align}
When $\frac{\vareps}{\sigma_m h}\leq\frac{1-\mu}{2||v||_\infty}$, \eqref{eq:proof_final} holds for arbitrary $\Dt>0$, hence the method is unconditionally stable. Otherwise, we need $\Dt$ to satisfy \eqref{eq:CFL} to have the conditional $\mu$-stability.
%%%%%%%%%%%%%%
\end{proof}

Next we will optimize the results in Theorem \ref{thm:mu_stable} in $\mu$ to maximize the unconditionally stable region and also the allowable time step size when the scheme
 is conditionally stable.  
%%%%%%%%%%%%%%%%%
% stability for IMEX1-DG1-S
%%%%%%%%%%%%%%%%
\begin{thm}[{\bf stability}]
%\textbf{(stability)}
\label{thm:stable}
The IMEX1-DG1-S scheme is unconditionally stable, if 
\begin{align}
\frac{\vareps}{\sigma_m h} \leq \frac{1}{2||v||_\infty}.
\end{align}
Otherwise, it is stable under the time step condition
\begin{align}
\Dt\leq\frac{2\vareps^2 h}{2\vareps ||v||_\infty-\sigma_mh}.\label{eq:CFL}
\end{align}
\end{thm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Optimization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
%[\bf Proof of Theorem  \ref{thm:stable}. ]
Based on the definition of $\mu$-stability and stability in Definition \ref{def:stab}, the results in Theorem \ref{thm:mu_stable} further imply that the IMEX1-DG1-S scheme is unconditionally stable if 
%If the IMEX1-DG1-S scheme is (unconditionally) $\mu$-stable for some $\mu\in[0,1]$,  it will be (unconditionally) stable. Hence, we can maximize $\lambda_0(\mu)$ in \eqref{eq:uncond-stable-region} to obtain the largest unconditionally stable region
\begin{align}
\frac{\varepsilon}{\sigma_m h}\leq\max_{\mu\in[0,1]}{\lambda_0(\mu) }= \max_{\mu\in[0,1]} \left(\frac{1-\mu}{2||v||_\infty}\right)=\frac{1}{2||v||_\infty}.
\end{align}
When $\frac{\vareps}{\sigma_m h}>\frac{1}{2||v||_\infty}$, the scheme is conditionally stable under the following time step restriction
% a finite time step restriction is needed. To maximize this time step restriction, we maximize $\tau_0(\mu)$:
\begin{align}
\Dt\leq\max_{\mu\in[0,1]}\tau_0(\mu)=\max_{\mu\in[0,1]}\left(\frac{2\vareps^2 h}{2\vareps ||v||_\infty-(1-\mu)\sigma_mh}\right)
=\frac{2\vareps^2 h}{2\vareps ||v||_\infty-\sigma_mh}.
\end{align}
%%%%%%%%%
\end{proof}

%%%%%
% General meshes
%%%%
\begin{rem}
\BL{ In general, one can assume the mesh is regular, namely,  there exists $\delta>0$ such that  $h_i/h\leq\delta, \forall i$ during the mesh refinement. The stability results in Theorems \ref{thm:mu_stable}-\ref{thm:stable} can be modified accordingly by replacing $||v||_\infty$ with  $||v||_\infty/\delta$.
}
\end{rem}

%%%%%%%%%%%%%%%%%%%%
% remark: stability for sigma_s = 0
%%%%%%%%%%%%%%%%%%%%
\begin{rem}
For a multiscale problem, it is possible to have subregions with $\sigma_s=0$ where the problem is purely transport. In this case,  $\sigma_m=0$, and 
our proofs above still hold. Specifically, the IMEX1-DG1-S scheme is always conditionally stable under the time step condition $\Dt\leq\frac{2\vareps^2 h}{2\vareps ||v||_\infty}=\frac{\vareps h}{||v||_\infty}$, and the unconditional stability is not expected.
\end{rem}
%\begin{rem}
%For a multiscale problem, it is possible that subregions with $\sigma_s=0$ exist. Actually, when $\sigma_m=0$, above proof can still be applied, and the IMEX1-DG1-S scheme is conditionally stable under the stability condition $\Dt\leq\frac{2\vareps^2 h}{2\vareps ||v||_\infty}$. The system is purely transport in the subregions where $\sigma_s=0$, and we should not expect unconditional stability in this case.
%\end{rem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Fourier analysis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Fourier Analysis for IMEX$k$-DG$k$-S scheme, $k=1, 2, 3$}\label{sec:fourier}

In this section, Fourier analysis is performed for the IMEX$k$-DG$k$-S scheme, $k=1, 2, 3$, when the schemes are applied to the one-group transport equation in slab geometry with $\Omega_v=[-1,1]$. Related, 
$\lgl f\rgl= 
%\int_{\Omega_v}F d\nu=
 \frac{1}{2}\int_{-1}^1 f(v)dv$, with $dv$ the standard  Lebesgue measure.
$16$ Gaussian quadrature points together with the weights are applied to the
discretization of the velocity space. 
As typical for Fourier analysis, it is assumed that the mesh is uniform and $\sigma_s(x)=\sigma_m>0, \; \forall x\in\Omega_x$. Motivated by that the  stability result for the IMEX1-DG1-S scheme in Section \ref{sec:energy} does not depend on $\sigma_a$, we further assume $\sigma_a=0$.
% \pzc{We also note that only $\sigma_m$ appeared in the stability condition for the IMEX1-DG1-S scheme.} 
 %$\int_{\Omega_v}d\nu = \frac{1}{2}\int_{\Omega_v}dv\frac{1}{2}\int_{\Omega_v}dv$. $16$ Gaussian quadrature points is applied to the discretization of the velocity space. 
 %Under this setting, Fourier (von Neumann) analysis is carried out.
Similar to \cite{peng2019stability}, %to perform the Fourier analysis, 
we first identify an invariant scaling structure of the amplification matrix. Then, by numerically solving an eigenvalue problem, we obtain the stability condition for IMEX$k$-DG$k$-S scheme, $k=1,2,3$. 


%We consider the one group transport equation with $\Omega_v=[-1,1]$ associated with the normalized Lebesgue measure $\int_{\Omega_v}d\nu = \frac{1}{2}\int_{\Omega_v}dv$. $16$ Gaussian quadrature points is applied to the discretization of the velocity space. Under this setting, Fourier (von Neumann) analysis is carried out.
%Similar to \cite{peng2019stability}, to perform the Fourier analysis, we first find an invariant scaling structure of the amplification matrix. Then, by numerically solving an eigenvalue problem, we obtain the stability condition for IMEX$k$-DG$k$-S scheme, $k=1,2,3$. We use the IMEX1-DG$k$-S scheme as an example to demonstrate the details.

\medskip
\noindent {\textbf{Setup of the Fourier analysis:} } 
%Motivated by the stability condition of the IMEX1-DG1-S scheme in Section \ref{sec:energy} in that the results do not depend on $$\sigma_a$, we assume $\sigma_a=0$, and $\sigma_s(x)=\sigma_m$ with some positive constant $\sigma_m$.    namely, the results
%we show that the stability condition of the IMEX1-DG1-S scheme can be determined by the minimum value of $\sigma_s(x)$, and $\sigma_a(x)$ has no contribution. Inspired by this, we assume a constant scattering coefficient $\sigma_s(x)\equiv\sigma_m$, a zero absorption coefficient $\sigma_a(x)=0$, uniform mesh and periodic boundary conditions. 
We will use the IMEX1-DG$k$-S scheme as an example to demonstrate the setup. 
%For IMEX$r$-DG$k$-S scheme, 
On the element $I_m$, the numerical solutions can be expanded as
\begin{align}
\rho_h^n(x)=\sum_{l=0}^{k-1}\rho^n_{ml}\phi_{l}^m(x),\quad g_{h,j}^n(x)=\sum_{l=0}^{k-1}g^n_{j,ml}\phi^{m}_l(x),\;\forall x\in I_m
\end{align}
where $\phi_l^{m}(x)=\phi_l\left( \frac{x-x_m}{h_m/2}\right)$, $\phi_l(x)$ is the $l$-th order  Legendre polynomial on $[-1, 1]$. Let ${\boldsymbol{\rho} }_m^n=(\rho_{m0}^n,\dots,\rho_{m\;k-1}^n)^T$ and ${\bf{g} }_{jm}^n=(g^n_{j,m0},\dots,g^n_{j,m\;k-1})^T$.

 
Take the Fourier anstaz ${\boldsymbol{\rho}}_m^n=\exp(\mathcal{I}\kappa x_m){\boldsymbol{\widehat{\rho}}}^n$ and ${\bf{g}}_{jm}^n=\exp(\mathcal{I}\kappa x_m){\bf{\widehat{g}}}_j^n$ (with $\mathcal I^2=-1$), and 
%where $x_m=mh$.
plug  them into the IMEX1-DGk-S scheme, we obtain
\begin{align}
\label{eq:fourier_matrix_vector}
&\underbrace{
\left(
\begin{matrix}
h\widehat{M} 		  	&\Dt \omega_1 v_1 \widehat{D}^+ 		& \Dt \omega_2 v_2 \widehat{D}^+ 		&\dots 	& \Dt\omega_{N_v}v_{N_v}\widehat{D}^+\\
v_1 \Dt \widehat{D}^- 	& h(\vareps^2+\sigma_m\Dt) \widehat{M} 	& 0 						&\dots 	& 0 \\
v_2 \Dt \widehat{D}^- 	& 0						&  h(\vareps^2+\sigma_m\Dt) \widehat{M}	&\dots 	& 0 \\
\vdots	  	& \vdots					& \vdots 					&\ddots	&\vdots\\
v_{N_v}\Dt \widehat{D}^-	& 0						& 0 						&\dots  	&  h(\vareps^2+\sigma_m\Dt) \widehat{M}
\end{matrix}
\right) }_{G_L}
\left(
\begin{matrix}
{\boldsymbol{\widehat{\rho}} }^{n+1} \\
{\bf{\widehat{g} }}_1^{n+1}\\
{\bf{\widehat{g} }}_2^{n+1}\\
\vdots\\
{\bf{\widehat{g}}}_{N_v}^{n+1}
\end{matrix}
\right)
\notag\\
=&\underbrace{\left(
\begin{matrix}
h\widehat{M} 		  	&0 		& 0	&\dots 	& 0\\
0	& \vareps^2 h\widehat{M}+\vareps\Dt \widehat{U}_1 	& 0 						&\dots 	& 0 \\
0	& 0						& \vareps^2 h\widehat{M}+\vareps\Dt \widehat{U}_2 &\dots 	& 0 \\
\vdots	  	& \vdots					& \vdots 					&\ddots	&\vdots\\
0	& 0						& 0 						&\dots  	&  \vareps^2 h\widehat{M}+\vareps\Dt \widehat{U}_{N_v} 
\end{matrix}
\right)}_{G_R}
\left(
\begin{matrix}
{\boldsymbol{\widehat{\rho}} }^{n} \\
{\bf{\widehat{g} }}_1^{n}\\
{\bf{\widehat{g} }}_2^{n}\\
\vdots\\
{\bf{\widehat{g}}}_{N_v}^{n}
\end{matrix}
\right).
\end{align}
Here, $\widehat{M}$, $\widehat{D}^{+}$, $\widehat{D}^-$ and $\widehat{U}$ are $k\times k$ matrices, and they are defined as follows.
\begin{subequations}
\begin{align}
&(\widehat{M})_{ij} = \frac{1}{2}\int_{-1}^{1}\phi_{i}(x)\phi_j(x) dx,\\
&(\widehat{D}^{-}(\xi)\;)_{ij}=- \int_{-1}^{1} \phi_j(x)\partial_x \phi_i(x)dx+ \phi_j(1) \phi_i(1)
-\exp({-\mathcal{I} \xi})\phi_j(1) \phi_i(-1),\\
&(\widehat{D}^{+}(\xi)\;)_{ij}=- \int_{-1}^{1} \phi_j(x)\partial_x \phi_i(x)dx+\exp({\mathcal{I} \xi}) \phi_j(-1) \phi_i(1)
-\phi_j(-1) \phi_i(-1),\\
%&(\widehat{U}_k(\xi)\;)_{ij}=(\widetilde{U}_k(\xi)\;)_{ij}-\sum_{k=1}^{N_v}\omega_k(\widetilde{U}_k(\xi)\;)_{ij},
&(\widehat{U}_{l}(\xi)\;)_{ij}=
\begin{cases}
v_{l}(\widehat{D}^{-}(\xi)\;)_{ij} -\sum_{l'=1}^{N_v}\omega_{l'} v_{l'}\big(\mathbbm{1}_{\{v_{l'}\geq0\}}(v_{l'})(\widehat{D}^{-}(\xi)\;)_{ij}+\mathbbm{1}_{\{v_{l'}<0\}}(v_{l'})(\widehat{D}^{+}(\xi)\;)_{ij}\big) ,\;\text{if}\;v_l\geq 0,\\
v_{l}(\widehat{D}^{+}(\xi)\;)_{ij}-\sum_{l'=1}^{N_v}\omega_{l'} v_{l'}\big(\mathbbm{1}_{\{v_{l'}\geq0\}}(v_{l'})(\widehat{D}^{-}(\xi)\;)_{ij}+\mathbbm{1}_{\{v_{l'}<0\}}(v_{l'})(\widehat{D}^{+}(\xi)\;)_{ij}\big),\;\text{if}\;v_l<0,
\end{cases}
\end{align}
\end{subequations}
where
$\xi=\kappa h$ is the discrete wave number, and $\mathbbm{1}_{S}(y)%=\begin{cases}
%1,\;y\in S,\\
%0,\;y\not\in S,
%\end{cases}
$
is the indicator function of the set $S$. 
Define block matrices 
\begin{align}
&{\bm{D} }^{-}=\left(v_1\widehat{D}^{-},\dots,v_{N_v}\widehat{D}^{-}\right)^T\in\mathbb{R}^{kN_v\times k},\;
{\bm{D} }^{+}=\left(\omega_1v_1\widehat{D}^{+},\dots,\omega_{N_v}v_{N_v}\widehat{D}^{+}\right)\in\mathbb{R}^{k\times kN_v},\notag\\
&{\bm{M} } = diag(\widehat{M},\dots,\widehat{M})\in\mathbb{R}^{kN_v\times kN_v},\;
{\bm{U} }= diag(\widehat{U}_1,\dots,\widehat{U}_{N_v})\in\mathbb{R}^{kN_v\times kN_v}.
\end{align}
Then, $G_L$ and $G_R$ can be rewritten as 
\begin{align}
G_L=\left(\begin{matrix}
h\widehat{M} & \Dt{\bm{D}}^+ \\
\Dt{\bm{D}}^-& h(\vareps^2+\sigma_m\Dt){\bm{M}}
\end{matrix}
\right)\;\;
\text{and}\;\;
G_R=\left(\begin{matrix}
h\widehat{M} & 0 \\
0& \vareps^2h{\bm{M}}+\vareps\Dt{\bm{U}}
\end{matrix}
\right),
\end{align}
With the amplification matrix as $\bm{G}^{(1,k)}=\bm{G}^{(1,k)}(\vareps,\sigma_m,h,\Dt; \xi)=G_L^{-1}G_R$ and ${\bf{V} }^{n}=\left({\boldsymbol{\widehat{\rho}} }^{n},{\bf{\widehat{g} }}_1^{n},{\bf{\widehat{g} }}_2^{n},\dots{\bf{\widehat{g}}}_{N_v}^{n}\right)^T$, \eqref{eq:fourier_matrix_vector} becomes ${\bf{V}}^{n+1}=G^{(1,k)}{\bf{V} }^n$. Similarly, the amplification matrix ${\bm{G}}^{(p,k)}$ of the  IMEX$p$-DG$k$-S scheme
can be derived. 
%Here, the dependence of ${\bm{G}}^{(p)}$ and ${\bm{G}}^{(p)}$ on $k$ is suppressed for simplicity.
To study the numerical stability, we will adopt the following principle. 
\begin{itemize}
\item[]
\noindent {\bf  Principle for Numerical Stability \cite{peng2019stability}:} {\em
For any given $\vareps, h, \Dt$, let the eigenvalues of $\bm{G}^{(p,k)}$ be $\lambda_i(\xi)$, $i=1,\dots, 2k$. Our scheme is said to be stable, if for all $\xi\in[0,2\pi]$, it satisfies either
	\begin{align}
(*)  \hspace{0.5in} &	\max_{i=1,\dots,2k}\{|\lambda_i(\xi)| \}<1,\quad\mbox{or}
	\label{fourier:stable_condition1}\\
(*) \hspace{0.5in}	&\max_{i=1,\dots,2k}\left\{|\lambda_i(\xi)| \right\}=1 \quad\text{and}\quad\bm{G}^{(p)}\quad\text{is diagonalizable}.
	\label{fourier:stable_condition2}
	\end{align}
	}
\end{itemize}
This principle is actually a necessary condition to guarantee the standard $L^2$ energy non-increasing. Before presenting the stability results, we first show an intrinsic scaling structure of the amplification matrices. 
%where
%\begin{align}
%(\widetilde{U}_k\;)_{ij}=
%\begin{cases}
%- \int_{-1}^{1} v_k\phi_j(x)\partial_x \phi_i(x)dx+v_k\phi_j(1) \phi_i(1)-v_k\exp(-{\mathcal{I}\xi})\phi_j(1) \phi_i(-1),\;\;&\text{if}\;v_k>0,\\
%- \int_{-1}^{1}v_k \phi_j(x)\partial_x \phi_i(x)dx+v_k\exp({\mathcal{I} \xi}) \phi_j(-1) \phi_i(1)-v_k\phi_j(-1) \phi_i(-1),\;\;&\text{if}\;v_k\leq0.
%\end{cases}
%\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Main findings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thm}\label{thm:fourier_invariant}
For any given $k\geq 1$  and $p=1, 2, 3$, the amplification matrix  ${\bm{G}^{(p,k)} }(\vareps,\sigma_m,h,\Dt;\xi)$ of the IMEX$p$-DG$k$-S  method  is similar to some matrix $\widehat{ \bm{G}}^{(p,k)}(\frac{\vareps}{\sigma_mh},\frac{\Dt}{\vareps h};\xi)$. In other words, the eigenvalues of ${\bm{G}^{(p,k)} }(\vareps,\sigma_m,h,\Dt;\xi)$ depend on $\vareps, h, \Dt, \sigma_m$ only  in terms of $\frac{\vareps}{\sigma_m h}$ and $\frac{\Dt}{\vareps h}$,  or equivalently, only in terms of $\frac{\vareps}{\sigma_mh}$ and $\frac{\vareps^2}{\sigma_m\Dt}=\frac{\vareps/(\sigma_m h)} {\Dt/(\vareps h)}$.
\end{thm}
\begin{proof}
We start  with $p=1$. 
%Then, we comment on how to generalize the proof to high order in time schemes. 
With  $J_m$ as the $m\times m$ identity matrix, one gets
\begin{align}
&{\bm{G}^{(1,k)} }=G_L^{-1}G_R\notag\\
&=
\left(
\left(
\begin{matrix}
\frac{\sigma_m}{\vareps}J_k & 0 \\
0& \frac{1}{\vareps^2 h}J_{kN_v}
\end{matrix}
\right)
\left(\begin{matrix}
h\widehat{M} & \Dt{\bm{D}}^+ \\
\Dt{\bm{D}}^-& h(\vareps^2+\sigma_m\Dt){\bm{M}}
\end{matrix}
\right)
\right)^{-1}
\left(
\begin{matrix}
\frac{\sigma_m}{\vareps}J_k & 0 \\
0& \frac{1}{\vareps^2 h}J_{kN_v}
\end{matrix}
\right)
\left(\begin{matrix}
h\widehat{M} & 0 \\
0& \vareps^2h{\bm{M}}+\vareps\Dt{\bm{U}}
\end{matrix}
\right)\notag\\
&=
\left(\begin{matrix}
\frac{\sigma_m h}{\vareps}\widehat{M} & \frac{\sigma_m\Dt}{\vareps}{\bm{D}}^+ \\
\frac{\Dt}{\vareps^2 h}{\bm{D}}^-& (1+\frac{\sigma_m\Dt}{\vareps^2 }){\bm{M}}
\end{matrix}
\right)^{-1}
\left(\begin{matrix}
\frac{\sigma_m h}{\vareps}\widehat{M} & 0 \\
0& {\bm{M}}+\frac{\Dt}{\vareps h}{\bm{U}}
\end{matrix}
\right).
\end{align}
Using the relations of
%\begin{subequations}
\begin{align*}
\left(\begin{matrix}
\sigma_mhJ_k & 0\\
0 & J_{kN_v}
\end{matrix}
\right)^{-1}
\left(\begin{matrix}
\frac{\sigma_m h}{\vareps}\widehat{M} & \frac{\sigma_m\Dt}{\vareps}{\bm{D}}^+ \\
\frac{\Dt}{\vareps^2 h}{\bm{D}}^-& (1+\frac{\sigma_m\Dt}{\vareps^2 }){\bm{M}}
\end{matrix}
\right)
\left(\begin{matrix}
\sigma_mhJ_k & 0\\
0 & J_{kN_v}
\end{matrix}
\right)
&=\left(\begin{matrix}
\frac{\sigma_m h}{\vareps}\widehat{M} & \frac{\Dt}{\vareps h}{\bm{D}}^+ \\
\frac{\sigma_m\Dt}{\vareps^2 }{\bm{D}}^-& (1+\frac{\sigma_m\Dt}{\vareps^2 }){\bm{M}}
\end{matrix}
\right),\\
%\text{and}\quad 
\left(\begin{matrix}
\sigma_mhJ_k & 0\\
0 & J_{kN_v}
\end{matrix}
\right)^{-1}
\left(\begin{matrix}
\frac{\sigma_m h}{\vareps}\widehat{M} & 0 \\
0& {\bm{M}}+\frac{\Dt}{\vareps h}{\bm{U}}
\end{matrix}
\right)
\left(\begin{matrix}
\sigma_mhJ_k & 0\\
0 & J_{kN_v}
\end{matrix}
\right)
&=\left(\begin{matrix}
\frac{\sigma_m h}{\vareps}\widehat{M} & 0 \\
0& {\bm{M}}+\frac{\Dt}{\vareps h}{\bm{U}}
\end{matrix}
\right),
\end{align*}
%\end{subequations}
we obtain
\begin{align}
&\left(\begin{matrix}
\sigma_m h J_k & 0\\
0 & J_{kN_v}
\end{matrix}
\right)^{-1}{\bm{G}}^{(1,k)}
\left(\begin{matrix}
\sigma_m h J_k & 0\\
0 & J_{kN_v}
\end{matrix}
\right)
%\notag\\
=\left(\begin{matrix}
\frac{\sigma_m h}{\vareps}\widehat{M} & \frac{\Dt}{\vareps h}{\bm{D}}^+ \\
\frac{\sigma_m\Dt}{\vareps^2 }{\bm{D}}^-& (1+\frac{\sigma_m\Dt}{\vareps^2 }){\bm{M}}
\end{matrix}
\right)^{-1}
\left(\begin{matrix}
\frac{\sigma_m h}{\vareps}\widehat{M} & 0 \\
0& {\bm{M}}+\frac{\Dt}{\vareps h}{\bm{U}}
\end{matrix}
\right)
\notag\\
&=\left(\begin{matrix}
\frac{\sigma_m h}{\vareps}\widehat{M} & \frac{\Dt}{\vareps h}{\bm{D}}^+ \\
\frac{\sigma_m h}{\vareps}\cdot\frac{\Dt}{\vareps h }{\bm{D}}^-& (1+\frac{\sigma_m h}{\vareps}\cdot\frac{\Dt}{\vareps h }){\bm{M}}
\end{matrix}
\right)^{-1}
\left(\begin{matrix}
\frac{\sigma_m h}{\vareps}\widehat{M} & 0 \\
0& {\bm{M}}+\frac{\Dt}{\vareps h}{\bm{U}}
\end{matrix}
\right)
=
\widehat{ \bm{G}}^{(1,k)}(\frac{\vareps}{\sigma_mh},\frac{\Dt}{\vareps h};\xi).
\end{align}
This implies that ${\bm{G}}^{(1,k)}$ is similar to $\widehat{ \bm{G}}^{(1,k)}(\frac{\vareps}{\sigma_mh},\frac{\Dt}{\vareps h};\xi)$.

The proof can be generalized to $p=2,3$ through the mathematical induction. To see this, let
${\bf V}^{n,(0)}={\bf V}^n$, ${\bf{V} }^{n,(l)}=\left({\boldsymbol{\widehat{\rho}} }^{n,(l)},{\bf{\widehat{g} }}_1^{n,(l)},{\bf{\widehat{g} }}_2^{n,(l)},\dots{\bf{\widehat{g}}}_{N_v}^{n,(l)}\right)^T$, $l=1, \dots, s$, we have
$${\bf V}^{n,(l)}=\sum_{q=0}^{l-1} {\bm{G}}^{(p,k)}_{lq}(\vareps,\sigma_m,h,\Dt;\xi) {\bf V}^{n,(q)},\; l=1,\dots,s,\;\;\text{and}\;\; {\bf V}^{n+1}={\bf V}^{n,(s)}.$$
With similar argument as for $p=1$, one can find a ${\bm{\widehat{G}}}^{(p,k)}_{lq}(\frac{\vareps}{\sigma_m h},\frac{\Dt}{\vareps h};\xi)$ such that $\forall\; l=1,\dots, s$,
$$
\left(\begin{matrix}
\sigma_m h J_k & 0\\
0 & J_{kN_v}
\end{matrix}
\right)^{-1}
{\bm{G}}^{(p,k)}_{lq}(\vareps,\sigma_m,h,\Dt;\xi)\left(\begin{matrix}
\sigma_m h J_k & 0\\
0 & J_{kN_v}
\end{matrix}
\right)={\bm{\widehat{G}}}^{(p,k)}_{lq}(\frac{\vareps}{\sigma_m h},\frac{\Dt}{\vareps h};\xi),\;\;q=0,\dots, l-1.
$$
For every ${\bm{G}}^{(p,k)}_{lq}(\vareps,\sigma_m,h,\Dt;\xi)$, exactly the same similar transformation is performed, hence, ${\bm{G}}^{(p,k)}$ is similar to some $\widehat{ \bm{G}}^{(p,k)}(\frac{\vareps}{\sigma_mh},\frac{\Dt}{\vareps h};\xi)$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Results of numerical Fourier analysis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\medskip
\noindent  \textbf{Fourier analysis results:} 
\BL{Based on Theorem \ref{thm:fourier_invariant} and the principle for numerical stability, the numerical stability results shall only depend on $\frac{\vareps}{\sigma_m h}$ and $\frac{\Dt}{\vareps h}$.  Set $\alpha=\log_{10}(\frac{\vareps}{\sigma_m h})$ and $\beta=\log_{10}(\frac{\Dt}{\vareps h})$.  For the IMEX$k$-DG$k$-S scheme, $k=1, 2, 3$, we numerically compute eigenvalues of the amplification matrix by uniformly sampling the discrete wave number $\xi\in
[0,2\pi]$ with spacing $\frac{2\pi}{100}$, $\beta\in[-5,4]$ and $\alpha\in[-5,5]$ with $\frac{1}{20}$ spacing. The stability results are presented in Figure \ref{fig:fourier}, with the white region being stable, and the black region being unstable. The main observations are summarized as follows, with $k=1, 2, 3$:
} 
%we numerically compute eigenvalues of the amplification matrix and get the stability region for the IMEX$k$-DG$k$-S scheme, $k=1, 2, 3$. The results are presented in Figure \ref{fig:fourier} in terms of  $\alpha=\log_{10}(\frac{\vareps}{\sigma_m h})$ and $\beta=\log_{10}(\frac{\Dt}{\vareps h})$. We uniformly sample the discrete wave number $\xi\in
%[0,2\pi]$ with spacing $\frac{2\pi}{100}$, $\beta\in[-5,4]$ and $\alpha\in[-5,5]$ with $\frac{1}{20}$ spacing. The main observations are summarized as follows, with $k=1, 2, 3$:
\begin{enumerate}
\item For some $\alpha_k$, the IMEX$k$-DG$k$-S scheme is unconditionally stable when $\alpha<\alpha_k$, i.e. when  $\frac{\vareps}{\sigma_m h}<C_k$. This %numerically
confirms the unconditional stability of the proposed schemes in the diffusive regime.
\item In the transport dominant regime with $\vareps/(\sigma_m h)=O(1)$,
%($h\ll \frac{\vareps}{\sigma_m}$), 
the stability region for the IMEX$k$-DG$k$-S is under a straight line $\beta=\beta_k$. In other words, in the transport dominant regime, the scheme is conditionally stable under a standard CFL condition
$$
\beta = \log_{10}{\frac{\Dt}{\vareps h}}\leq\beta_k\Leftrightarrow \Dt\leq \widehat{C}_k\vareps h.
$$
\item The IMEX$k$-DG$k$-S scheme is stable under the condition  $\beta\leq \mathcal{F}_k(\alpha)$, with some function $\mathcal{F}_k$. Based on this, we can further derive the stability condition $\Dt\leq \widetilde{\mathcal{F}}_k(\vareps,h,\sigma_m)$. The time step condition for the IMEX$k$-DG$k$-S schemes with $k=2,3$ in Section \ref{sec:numerical} is actually obtained through such  procedure.
\item The Fourier results for IMEX1-DG$1$-S scheme match well with the energy analysis results.
\end{enumerate}

We want to mention that the stability properties of the IMEX-DG-S schemes are qualitatively  similar to that for the IMEX-LDG schemes in \cite{peng2019stability} with the numerical weight $\omega=\exp(-\frac{\varepsilon}{\sigma_m h})$.
%%%%%%%%%%%%%%%%%%%
%\begin{rem}
%Though not shown in this paper, we numerically observe that the stability condition depends on the choice of the collocation points $\{v_j\}_{j=1}^{N_v}$. More specifically, similar observations can still be made when collocation points change, but the values of $C_k$, $\beta_k$ and the specific form of $\mathcal{F}_k$ depend on the choice of the collocation points.
%\end{rem}

%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \centering 
   \subfigure[IMEX$1$-DG$1$-S]
    { \includegraphics[width=0.31\linewidth]{./picture/imex1s.png} }
    \subfigure[IMEX$2$-DG$2$-S ]
  {    \includegraphics[width=0.31\linewidth]{./picture/imex2s.png}}   
  \subfigure[IMEX$3$-DG$3$-S]
 {      \includegraphics[width=0.31\linewidth]{./picture/imex3s.png}      }   
  \caption{Stability regions of the IMEX$k$-DG$k$-S methods, $k=1, 2, 3$. White: stable; black: unstable. $\alpha=\log_{10}(\frac{\vareps}{\sigma_m h})$ and $\beta=\log_{10}(\frac{\Dt}{\vareps h}).$}
  \label{fig:fourier}
\end{figure}
%%%%%%%%%%%%%%%%%%%











==> source/sec_stability_opt_general_k.tex <==
\section{Stability}
\label{sec:stability}
Plan for stability:\\
(1) Prove everything and do the optimization here. \\
(2) Prove uniform stability and accuracy in a second paper. \\
(3) Maybe, I can provide all the details in my thesis for now, and the decide. Finish numerical section first.

\subsection{Energy analysis for IMEX-1 scheme}
\begin{thm}
\end{thm}
\begin{proof}
Take $\testR=\rho_h^{n+1}$ in \eqref{eq:space_rho}, and take $\testG=\vareps^2 g_h^{n+1}$ in \eqref{eq:space_g}, then integrate \eqref{eq:space_g}  in $\Omega_v$, we have 
\begin{subequations}
\begin{align}
&\frac{1}{\Dt}(\rho_h^{n+1}-\rho_h^n,\rho_h^{n+1})+l_h(\lgl vg_h^{n+1}\rgl,\rho_h^{n+1})\notag\\
=&\frac{1}{2\Dt}(||\rho_h^{n+1}||^2-||\rho_h^n||^2+||\rho_h^{n+1}-\rho_h^n||^2)+l_h(\lgl vg_h^{n+1}\rgl,\rho_h^{n+1}) 
=-(\sigma_a\rho_h^n,\rho_h^{n+1}),
\label{eq:proof1-1}\\
&\frac{\vareps^2}{\Dt}\lgl(g_h^{n+1}-g_h^n,g_h^{n+1})\rgl+\vareps \lgl b_{h,v}(g_h^n,g_h^{n+1})\rgl-\lgl vd_h(\rho_h^{n+1}, g_h^{n+1})\rgl\notag\\
=&\frac{\vareps^2}{2\Dt}(|||g_h^{n+1}|||^2-|||g_h^n|||^2+|||g_h^{n+1}-g_h^n|||^2)+\vareps\lgl b_{h,v}(g_h^n,g_h^{n+1})\rgl
-d_h(\rho_h^{n+1}, \lgl vg_h^{n+1}\rgl)\notag\\
=& -\lgl (\sigma_s g_h^{n+1},g_h^{n+1})\rgl-\lgl (\sigma_a g_h^{n},g_h^{n+1})\rgl = -|||g_h^{n+1}|||_s^2-\lgl (\sigma_a g_h^{n},g_h^{n+1})\rgl.
\label{eq:proof1-2}
\end{align}
\end{subequations}

With Lemma \ref{lem:adjoint_relation}, we have $l_h(\lgl vg_h^{n+1}\rgl,\rho_h^{n+1})-d_h(\rho_h^{n+1},\lgl vg_h^{n+1}\rgl)=0$. Based on this, and sum up \eqref{eq:proof1-1} and \eqref{eq:proof1-2}, we obtain
\begin{align}
&\frac{1}{2\Dt}( ||\rho_h^{n+1}||^2+\vareps^2|||g_h^{n+1}|||^2-||\rho_h^n||^2-\vareps^2|||g_h^n|||^2)
+\frac{1}{2\Dt}(||\rho_h^{n+1}-\rho_h^n||^2+\vareps^2|||g_h^{n+1}-g_h^n|||^2)
\notag\\
&+(\sigma_a\rho_h^n,\rho_h^{n+1})+\lgl (\sigma_a g_h^{n},g_h^{n+1})\rgl+|||g_h^{n+1}|||_s^2+\vareps\lgl b_{h,v}(g_h^n,g_h^{n+1})\rgl=0.
\label{eq:proof1}
\end{align}
Similar to \cite{OurAnalysisPaper}, we split $|||g_h^{n+1}|||_s^2$ into 
\begin{align}
\label{eq:proof_split}
|||g_h^n|||_s^2
=\mu|||g_h^n|||_s^2+ (1-\mu)\Big(\frac{1}{2}|||g_h^n|||_s^2-\frac{1}{2}|||g_h^{n-1}|||_s^2
+\frac{1}{4}|||g_h^n-g_h^{n-1} |||_s^2 + \frac{1}{4}|||g_h^n+g_h^{n-1} |||_s^2\Big).
 \end{align}
 Similar to \cite{OurAnalysisPaper} and \cite{jang2014analysis}, we split $\lgl b_{h,v}(g_h^n,g_h^{n+1})\rgl$ as $\lgl b_{h,v}(g_h^n-g_h^{n+1},g_h^{n+1})\rgl+\lgl b_{h,v}(g_h^{n+1},g_h^{n+1})\rgl$, and for each term, based on Young's inequalities and inverse inequalities, we have following estimations:
\begin{align}
&\lgl \bh(g_h^n,g_h^n)\rgl =\left\lgl\sum_i\frac{|v|}{2}[g_h^n]_\iL^2 \right\rgl,\label{eq:upwind}\\
&| \lgl \bh(g_h^{n}-g_h^{n-1} ,g_h^n) \rgl |\notag\\
&\leq (\frac{\theta}{\sigma_m}+\eta) |||g_h^n-g_h^{n-1}|||^2+\frac{\sigma_m}{4\theta}\left\lgl \sum_i \int_{I_i} (v\partial_x g_h^n)^2 dx\right\rgl+\frac{C_{inv} }{4\eta h}\sum_i \left\lgl (v[g_h^n]_\iL)^2\right \rgl\notag\\
&\leq (\frac{\theta}{\sigma_m}+\eta) |||g_h^n-g_h^{n-1}|||^2 +\frac{\widehat{C }_{inv}  ||v^2||_\infty}{4\theta h^2} \left(\sigma_m ||| g_h^n|||^2\right) +\frac{C_{inv} ||v||_{\infty} }{2\eta h}\left\lgl \frac{|v|}{2}\sum_i [g_h^n]_\iL^2  \right\rgl
\notag\\
&\leq(\frac{\theta}{\sigma_m}+\eta) |||g_h^n-g_h^{n-1}|||^2 +\frac{\widehat{C }_{inv}  ||v^2||_\infty}{4\theta h^2} |||g_h^n|||_s^2
+\frac{C_{inv} ||v||_{\infty} }{2\eta h}\left\lgl \frac{|v|}{2}\sum_i [g_h^n]_\iL^2  \right\rgl,
\label{eq:upwind_jump}
\end {align}
where $\theta$ and $\eta$ are positive parameters, and will be determined later.

Substitute \eqref{eq:proof_split}, \eqref{eq:upwind} and \eqref{eq:upwind_jump} into \eqref{eq:proof1}, we get
\begin{align}
&\frac{1}{2\Dt}( E_{\mu,h}^{n+1}-E_{\mu,h}^n)+\frac{1}{2\Dt}||\rho_h^{n+1}-\rho_h^n||^2
+(\frac{\vareps^2}{2\Dt}+\frac{1-\mu}{4}\sigma_m - \frac{\theta}{\sigma_m}-\eta)|||g_h^{n+1}-g_h^n|||^2\notag\\
&+\frac{1-\mu}{4}|||g_h^{n+1}+g_h^n|||_s^2+(\mu-\frac{\widehat{C}_{inv}||v^2||_\infty }{4\theta h^2})|||g_h|||_s^2+\vareps(1-\frac{C_{inv}||v||_\infty}{2\eta h})\lgl \sum_{i}\lgl\frac{|v|}{2}[g_h^{n+1}]^2\rgl
\leq 0.
\end{align}

In order to guarantee $E_{\mu,h}^{n+1}\leq E_{\mu,h}^n$, we require 
\begin{subequations}
\begin{align}
&\frac{\vareps^2}{2\Dt}+\frac{1-\mu}{4}\sigma_m - \frac{\theta}{\sigma_m}-\eta\geq 0,\\
&\mu-\frac{\widehat{C}_{inv}||v^2||_\infty }{4\theta h^2}\geq 0,\label{eq:proof_l2}\\
&1-\frac{C_{inv}||v||_\infty}{2\eta h}\geq 0.\label{eq:proof_l3}
\end{align}
\end{subequations}
We choose $\frac{\theta}{\sigma_m}=\eta=\frac{1}{2}\left(\frac{\vareps^2}{2\Dt}+\frac{1-\mu}{4}\sigma_m\right)$. Substitute this into \eqref{eq:proof_l2} and \eqref{eq:proof_l3}
\begin{subequations}
\begin{align}
&\frac{\vareps^2}{\Dt}\geq\frac{2\vareps^2 \widehat{C}_{inv}||v^2||_\infty-(1-\mu)\mu\sigma_m^2h^2}{2\vareps^2\sigma_m\mu h^2},\\
&\frac{\vareps^2}{\Dt}\geq\frac{C_{inv}||v||_\infty-(1-\mu)h }{4\sigma_m h}.
\end{align}
\end{subequations}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{proof}

